Enhanced Anomaly Detection in Industrial Control Systems aided by Machine Learning

Traditional intrusion detection systems (IDSs) often rely on either network traffic or process data, but this single-source approach may miss complex attack patterns that span multiple layers within industrial control systems (ICSs) or persistent threats that target different layers of operational technology systems. This study investigates whether combining both network and process data can improve attack detection in ICSs environments. Leveraging the SWaT dataset, we evaluate various machine learning models on individual and combined data sources. Our findings suggest that integrating network traffic with operational process data can enhance detection capabilities, evidenced by improved recall rates for cyber attack classification. Serving as a proof-of-concept within a limited testing environment, this research explores the feasibility of advancing intrusion detection through a multi-source data approach in ICSs. Although the results are promising, they are preliminary and highlight the need for further studies across diverse datasets and refined methodologies.

==> paper.bbl.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}

\bibitem{iec62443}
Industrial Communication Networks --  part 3-3: System security requirements and security levels,
  \url{https://webstore.iec.ch/publication/6028}.

\bibitem{sklearn_pca}
{Sklearn Document}, 
  \url{https://scikit-learn.org},
  [Online; accessed Apr. 2024]

\bibitem{abdi2010principal}
Abdi, H., Williams, L.J.: Principal component analysis. Wiley interdisciplinary
  reviews: computational statistics  \textbf{2}(4),  433--459 (2010)

\bibitem{ackerman2021industrial}
Ackerman, P.: Industrial Cybersecurity: Efficiently monitor the cybersecurity
  posture of your ICS environment. Packt Publishing Ltd (2021)

\bibitem{alexander2020mitre}
Alexander, O., Belisle, M., Steele, J.: Mitre att\&ck for industrial control
  systems: Design and philosophy. The MITRE Corporation: Bedford, MA, USA
  \textbf{29} (2020)

\bibitem{breiman2001random}
Breiman, L.: Random forests. Machine Learning  \textbf{45}(1),  5--32 (2001).


\bibitem{chawla2002smote}
Chawla, N.V., Bowyer, K.W., Hall, L.O., Kegelmeyer, W.P.: Smote: synthetic
  minority over-sampling technique. Journal of artificial intelligence research
   \textbf{16},  321--357 (2002)

\bibitem{cortes1995svm}
Cortes, C., Vapnik, V.: Support vector networks. Machine Learning
  \textbf{20}(3),  273--297 (1995). 

\bibitem{cyber_report_2023}
DNV: Cyber priority 2023. Tech. rep., DNV AS, accessed: 1. Desember 2023

\bibitem{galloway2012introduction}
Galloway, B., Hancke, G.P.: Introduction to industrial control networks. IEEE
  Communications surveys \& tutorials  \textbf{15}(2),  860--880 (2012)

\bibitem{GAMAGE2020102767}
Gamage, S., Samarabandu, J.: Deep learning methods in network intrusion
  detection: A survey and an objective comparison. Journal of Network and
  Computer Applications  \textbf{169},  102767 (2020).

\bibitem{goh2016}
Goh, J., Adepu, S., Tan, M., Lee, Z.S.: Anomaly detection in cyber physical
systems using recurrent neural networks. In: 2017 IEEE 18th International
Symposium on High Assurance Systems Engineering (HASE). pp. 140--145 (2017)

\bibitem{garcia2009anomaly}
Garcia-Teodoro, P., Diaz-Verdejo, J., Maci{\'a}-Fern{\'a}ndez, G., V{\'a}zquez,
  E.: Anomaly-based network intrusion detection: Techniques, systems and
  challenges. computers \& security  \textbf{28}(1-2),  18--28 (2009)

\bibitem{hastie2009elements}
Hastie, T., Tibshirani, R., Friedman, J.: The Elements of Statistical Learning:
  Data Mining, Inference, and Prediction. Springer Series in Statistics,
  Springer New York (2009). \doi{10.1007/978-0-387-84858-7},


\bibitem{hutchins2011intelligence}
Hutchins, E.M., Cloppert, M.J., Amin, R.M., et~al.: Intelligence-driven
  computer network defense informed by analysis of adversary campaigns and
  intrusion kill chains. Leading Issues in Information Warfare \& Security
  Research  \textbf{1}(1), ~80 (2011)

\bibitem{jadidi2022automated}
Jadidi, Z., Foo, E., Hussain, M., Fidge, C.: Automated detection-in-depth in
  industrial control systems. The International Journal of Advanced
  Manufacturing Technology  \textbf{118}(7),  2467--2479 (2022)



\bibitem{konijn2022multi}
Konijn, J.P.: Multi-domain Cyber-attack Detection in Industrial Control
  Systems. Master's thesis, University of Twente (2022)

\bibitem{kumar2017knn}
Kumar, S., Choudhary, G., Kumar, Y.: An analysis of the k-nearest neighbor
  technique for the intrusion detection system. In: 2017 IEEE International
  Conference on Computing and Communication Technologies for Smart Nation
  (IC3TSN). pp. 325--329 (2017). 
  
  \bibitem{kravchik2018}
  Kravchik, M., Shabtai, A.: Detecting cyberattacks in industrial control systems
  using convolutional neural networks, Proceedings of the 2018 Workshop on Cyber-Physical Systems Security and Privacy, pp. 72-83 (2018)

\bibitem{swat_technical_report}
iTrust Labs: Swat technical report,
  \url{https://itrust.sutd.edu.sg/itrust-labs\_datasets/dataset\_info/}

\bibitem{liu2019cnn}
Liu, X., Zhu, J., Li, L.: 1d convolutional neural networks and applications: A
  comprehensive review. Journal of Neural Networks  (2019).


\bibitem{mishra2019ml_ids}
Mishra, P., Varadharajan, V., Tupakula, U., Pilli, E.: A detailed investigation
  and analysis of using machine learning techniques for intrusion detection.
  IEEE Communications Surveys \& Tutorials  \textbf{21}(1),  686--728 (2019).


\bibitem{8386762}
Mishra, P., Varadharajan, V., Tupakula, U., Pilli, E.S.: A detailed
  investigation and analysis of using machine learning techniques for intrusion
  detection. IEEE Communications Surveys and Tutorials  \textbf{21}(1),
  686--728 (2019). 

\bibitem{patcha2007overview}
Patcha, A., Park, J.M.: An overview of anomaly detection techniques: Existing
  solutions and latest technological trends. Computer networks
  \textbf{51}(12),  3448--3470 (2007)

\bibitem{quinlan1993c45}
Quinlan, J.R.: {C4.5}: Programs for Machine Learning. Morgan Kaufmann (1993)

\bibitem{shalyga2018anomaly}
Shalyga, D., Filonov, P., Lavrentyev, A.: Anomaly detection for water treatment
  system based on neural network with automatic architecture optimization
  (2018)

\bibitem{smith1998fuzzy_ann}
Smith, J.W., Wilson, M.L.: An intelligent hybrid system for pattern
  recognition: Integrating fuzzy c-means clustering with neural networks.
  Neural Networks Journal  (1998). 

\bibitem{stouffer2022guide}
Stouffer, K., Pease, M., Tang, C., Zimmerman, T., Pillitteri, V., Lightman, S.:
  Guide to operational technology (ot) security. National Institute of
  Standards and Technology: Gaithersburg, MD, USA  (2022).
  \doi{10.6028/NIST.SP.800-82r3}

\bibitem{sullivan2016components}
Sullivan, D., Luiijf, E., Colbert, E.J.: Components of industrial control
  systems. Springer (2016)

\bibitem{itrust}
of~Technology, S.U., (SUTD), D.: {iTrust Labs}.
  \url{https://itrust.sutd.edu.sg/itrust-labs-home/itrust-labs\_swat/},
  accessed: Accessed: 6. Oct. 2023

\end{thebibliography}

